Joint 3D Reconstruction of a Static Scene and Moving Objects

We present a technique for simultaneous 3D reconstruction of static regions and rigidly moving objects in a scene. An RGB-D frame is represented as a collection of features, which are points and planes. We classify the features into static and dynamic regions and grow separate maps, static and object maps, for each of them. To robustly classify the features in each frame, we fuse multiple RANSAC-based registration results obtained by registering different groups of the features to different maps, including (1) all the features to the static map, (2) all the features to each object map, and (3) subsets of the features, each forming a segment, to each object map. This multi-group registration approach is designed to overcome the following challenges: scenes can be dominated by static regions, making object tracking more difficult; and moving object might have larger pose variation between frames compared to the static regions. We show qualitative results from indoor scenes with objects in various shapes. The technique enables on-the-fly object model generation to be used for robotic manipulation.

==> abstract.tex <==
\begin{abstract}

We present a method for simultaneous 3D reconstruction of static regions and rigidly moving objects in a scene. An RGB-D frame is represented as a collection of features, that are points and planes. The features are grouped into static and dynamic regions, where we grow separate 3D maps for each of them. We propose a multi-stage registration scheme used to distinguish features coming from regions with different motion patterns. In the first stage, all features of the frame are registered with both of the static and object maps following a RANSAC procedure. In the second stage, we employ a feature grouping approach in order to overcome the following challenges: (i) scenes can be dominated by static regions, making object tracking more difficult; and (ii) moving object might have larger pose variation between frames compared to the static regions. We represent dynamic regions with a set of segments that are disjoint subsets of features. We carry out an appearance search followed by a geometrical verification between the segments of the frame and the segments in the object map. The final pose of the moving object is obtained after a refinement between all features in the object map and the features in the frame, where the estimated pose from geometric verification is used as a prediction. The multi-stage scheme provides accurate pose estimates and enables classification of features into static and moving regions. We show qualitative results from indoor scenes with objects in various shapes. The technique enables on-the-fly object model generation to be used for robotic manipulation.

\end{abstract}

%\begin{keywords}
%\textit{SLAM, Object modeling, Object tracking}
%\end{keywords}

